A linear programming approach to general dataflow process network verification and dimensioning

In this paper, we present linear programming-based sufficient conditions, some of them polynomial-time, to establish the liveness and memory boundedness of general dataflow process networks. Furthermore, this approach can be used to obtain safe upper bounds on the size of the channel buffers of such a network.

==> eptcsdata.tex <==
\providecommand{\firstpage}{115}
\providecommand{\publicationstatus}{Bliudze, Bruni, Grohmann, Silva (Eds.):\\Third Interaction and Concurrency Experience (ICE 2010)\\
EPTCS 38, 2010, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.38.11}{10.4204/EPTCS.38.11}}
\pdfoutput=1

